Fermion mass and mixing pattern in a minimal T7 flavor 331 model

We present a model based on the $SU(3)_{C}\otimes SU(3)_{L}\otimes U(1)_{X}$ gauge symmetry having an extra $T_{7}\otimes Z_{2}\otimes Z_{3}\otimes Z_{14} $ flavor group, which successfully describes the observed SM fermion mass and mixing pattern. In this framework, the light active neutrino masses arise via double seesaw mechanism and the observed charged fermion mass and quark mixing hierarchy is a consequence of the $Z_{2}\otimes Z_{3}\otimes Z_{14}$ symmetry breaking at very high energy. In our minimal $T_{7}$ flavor 331 model, the spectrum of neutrinos includes very light active neutrinos as well as heavy and very heavy sterile neutrinos. The obtained physical observables for both quark and lepton sectors are compatible with their experimental values. The model predicts the absence of leptonic Dirac CP violating phase.

==> convention.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% Macros for References %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% [ roman version ] %%%%%%%%%%

\def\2tvec#1#2{
\left(
\begin{array}{c}
#1  \\
#2  \\   
\end{array}
\right)}


\def\mat2#1#2#3#4{
\left(
\begin{array}{cc}
#1 & #2 \\
#3 & #4 \\
\end{array}
\right)
}


\def\Mat3#1#2#3#4#5#6#7#8#9{
\left(
\begin{array}{ccc}
#1 & #2 & #3 \\
#4 & #5 & #6 \\
#7 & #8 & #9 \\
\end{array}
\right)
}

\def\3tvec#1#2#3{
\left(
\begin{array}{c}
#1  \\
#2  \\   
#3  \\
\end{array}
\right)}

\def\4tvec#1#2#3#4{
\left(
\begin{array}{c}
#1  \\
#2  \\   
#3  \\
#4  \\
\end{array}
\right)}

%%%%%%%%
\def\5tvec#1#2#3#4#5{
\left(
\begin{array}{c}
#1  \\
#2  \\
#3  \\
#4  \\
#5  \\
\end{array}
\right)}
%%%%%%%%



\def\L{\left}
\def\R{\right}

\def\pl{\partial}

\def\lra{\leftrightarrow}


%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% End of Macros %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



